Sensitivity of the SHiP experiment to Heavy Neutral Leptons

Heavy Neutral Leptons (HNLs) are hypothetical particles predicted by many extensions of the Standard Model. These particles can, among other things, explain the origin of neutrino masses, generate the observed matter-antimatter asymmetry in the Universe and provide a dark matter candidate. The SHiP experiment will be able to search for HNLs produced in decays of heavy mesons and travelling distances ranging between $\mathcal{O}(50\text{ m})$ and tens of kilometers before decaying. We present the sensitivity of the SHiP experiment to a number of HNL's benchmark models and provide a way to calculate the SHiP's sensitivity to HNLs for arbitrary patterns of flavour mixings. The corresponding tools and data files are also made publicly available.

==> LetterEditor.tex <==
Dear Editor

We are asking to dismiss the Referee 2. 

The referee report contains  two claims that are subjective and unjustified 
and make us us believe that the Referee 2 is biased. 

1. The Referee 2 suggests that a paper like this  should not be published in a journal (JHEP or similar) but should exist in a form of a preprint/SHiP note. 

We disagree with this opinion. Sensitivity estimates play a central role for any planned experiment. 
In the present  paper we present a number of new original results in this direction.


1. New Monte Carlo simulations based on the official collaboration software
that was significantly extended and developed, including improved description
of the signal, background and detector.
Some of the  results are also cross-checked by analytical computations. 

The resulting sensitivity is significantly different from the one published by the collaboration previously. 
 
 2. In addition we presented a new method that allows to estimate the sensitivity for any combination of HNL parameters -- something that has never been done before and that can be used by other Intensity Frontier experiments, for example.

It is our firm belief that such results should be peer reviewed and published in a respectable journal like JHEP. 


Long and detailed report of the Referee 1 with both questions and suggestions confirms that we are right. 

2. The Referee 2 expressed a strong opinion about production fraction of $B_c$ mesons at SHiP energies. He claims that treating this quantity as a source of major theoretical uncertainty is misleading. 
 To justify this claim the Referee 2 refers to the paper of 1998. 

However, this paper provides also a prediction of the production fraction of $B_c$  at the LHC energies This prediction is off by about an order of magnitude.  It seems completely unjustified to consider this 
work as a definite answer to the question, such that talking about theoretical uncertainty becomes
“misleading”.

After that paper of 1998 making wrong prediction for the LHC, there is no reference
that claims to reliably resolve this question theoretically. Corresponding measurements
are also absent. 

We want to stress that we have consulted many experts on the subject, authors of PYTHIA and other Monte Carlo generating QCD tools. It is their common opinion that the production fraction is not known and has not been reliably computed by anyone.  The real answer is somewhere between maximal (LHC) and minimal value".
 
We added the discussion of the 1998 paper. 

However, in the situation described above the Referee 2  expresses a very
strong opinion about the presentation of the results and moreover, insists
that the paper can not be published unless we remove the treatment of the 
production fraction of $B_c$ as a source of major uncertainty. 


We believe that this is completely unjustified and voluntary.


We ask the Editor to dismiss the Referee 2.



==> LetterReferees.tex <==
We thank the Referees for providing valuable comments on our manuscript.
In the updated version of the manuscript we have addresses all comments by both Referees (our changes are marked in blue to facilitate the reading):
\begin{enumerate}
    \item We have updated introduction to  clarifying the changes since the original technical proposal and added references about the SHiP background studies
    \item Following the comments 1-6 of the Referee 1, we rewrote the beginning of Section 4, in particular changed Eqs. (4.2)-(4.5)
     in order to make the presentation clear and to address all the questions raised by the Referee.
    \item Answering the request of Referee 1 we have described the sample size used in Monte Carlo simulations
    \item We have updated the references and corrected various typos (we thank the Referee 1 for providing the list of changes)
    \item Following the request of Referee 2 we expanded discussion of the production fraction of $B_c$ meson in Section 2, describing previous theoretical computations (and citing relevant references, including those, provided by the Referee II). We argued that existing theoretical predictions do not coincide with measurements at LHC energies and therefore cannot be trusted at SHiP energies.
    We also updated captions accordingly
\end{enumerate}
